Position-Blind Ptychography: Viability of image reconstruction via data-driven variational inference

In this work, we present and investigate the novel blind inverse problem of position-blind ptychography, i.e., ptychographic phase retrieval without any knowledge of scan positions, which then must be recovered jointly with the image. The motivation for this problem comes from single-particle diffractive X-ray imaging, where particles in random orientations are illuminated and a set of diffraction patterns is collected. If one uses a highly focused X-ray beam, the measurements would also become sensitive to the beam positions relative to each particle and therefore ptychographic, but these positions are also unknown. We investigate the viability of image reconstruction in a simulated, simplified 2-D variant of this difficult problem, using variational inference with modern data-driven image priors in the form of score-based diffusion models. We find that, with the right illumination structure and a strong prior, one can achieve reliable and successful image reconstructions even under measurement noise, in all except the most difficult evaluated imaging scenario.

==> sections/3_02_posrecovery_analysis.tex <==
\rev
\subsection{On the convergence of the position recovery problem}

We provide a theoretical treatment of the possibility of correct position recovery, which will ultimately motivate our choice of probe function discussed in \cref{sec:problem-setup:probe-functions}. To this end, we re-frame the measurement likelihood
%, which calculates the difference between the ground-truth and estimated diffraction patterns,
as a comparison between the autocorrelation function of the ground-truth probe-object product at the correct position $r$
%, which we denote as $r$ here,
and the autocorrelation function of the probe-object product at an estimated position $\hat{r}$. For notational simplicity, we treat a one-dimensional variant of the problem, but our arguments also hold in higher dimensions. We first make the following assumption:
%
\begin{ass}\label{ass:position-recovery-image-known}
    The image $x$ is already known and only the correct recovery of the position $\hat{r} = r$ is required.
\end{ass}
%
While \cref{ass:position-recovery-image-known} is different from the actual joint image-position recovery problem we would like to solve here, it nonetheless allows us insights into the sub-problem of position recovery. We are interested in under which conditions on the object $x$ and the probe $p$ the loss induced by the measurement likelihood is convex with respect to the estimated position $\hat{r}$. If convexity can be shown, a unique global minimum exists and a gradient-based scheme can attain correct position recovery.
First, we rewrite the Gaussian measurement likelihood equivalently \eqref{eq:likelihood-gaussian} as follows.
\begin{align}
    \log p(y|x,\hat{r})
        &\propto \left\lVert y - |A(\hat{r}, x)|^2 \right\rVert_2^2\\
        &= \left\lVert |A(r, x)|^2 - |A(\hat{r}, x)|^2 \right\rVert_2^2 \\
        &= \left\lVert \mathcal{F}(|A(r, x)|^2 - |A(\hat{r}, x)|^2)  \right\rVert_2^2 \\
        &= \left\lVert \mathcal{F}(|A(r, x)|^2) - \mathcal{F}(|A(\hat{r}, x)|^2)  \right\rVert_2^2 \\
\end{align}
where the first equality used the measurement likelihood definition, the second used the definition of the measurement $y$, the third used the fact that the Fourier transform $\mathcal{F}$ is unitary, and the final equality uses the linearity of $\mathcal{F}$. Recall that the operator $\mathcal{A}$ is defined as the Fourier transform of the element-wise product of the probe $p$ and the object $x$ shifted to position $r$,\todo{TR: are we already in 1D here? SW: yes. should be made clearer beforehand that we do this for easier notation}
%
\begin{equation}
    A(r,x) = \mathcal{F}(p(t)x(t-r)) = \mathcal{F}(z_r),
\end{equation}
%
where we introduced the variable $z_r$ for the inner quantity as a notational aid.
%
% \begin{equation}
%     z_r(t) := p(t)x(t-r) \quad \Rightarrow A(r,x) = \mathcal{F}(z_r).
% \end{equation}
%
Then, due to Wiener \& Khinchin \cite{todowienerkhinchin}, we can equivalently write the likelihood in terms of the auto-correlations of $z_r$ and $z_{\hat{r}}$, where we denote the auto-correlation of $z_r$ as $(z_r \star z_r)$:\todo[inline]{TR: what is $n$ here? SW: just the dimensionality of $x$, should introduce this}
%
\begin{align}
    \log p(y|x,\hat{r})
    &= \left\lVert \mathcal{F}(|A(r, x)|^2) - \mathcal{F}(|A(\hat{r}, x)|^2)  \right\rVert_2^2 \\
    &= \left\lVert (z_{r} \star z_{r}) - (z_{\hat{r}} \star z_{\hat{r}})  \right\rVert_2^2 \\
    &= \sum_{\ell=0}^{n-1} \left| \sum_{t=0}^{n-1} z_r(t)\overline{z_r(t-\ell)} - \sum_{t=0}^{n-1} z_{\hat{r}}(t) \overline{z_{\hat{r}}(t-\ell)} \right|^2 \\
   &= \sum_{\ell=0}^{n-1} \left| \sum_{t=0}^{n-1} z_r(t)\overline{z_r(t-\ell)} - z_{\hat{r}}(t) \overline{z_{\hat{r}}(t-\ell)} \right|^2 \\
   &= \sum_{\ell=0}^{n-1} \left| \sum_{t=0}^{n-1} p(t)x(t-r)\overline{p(t-\ell)x(t-r-\ell)} - p(t)x(t-\hat{r}) \overline{p(t-\ell)x(t-\hat{r}-\ell)} \right|^2 \\
   &= \sum_{\ell=0}^{n-1} \left| \sum_{t=0}^{n-1} p(t)\overline{p(t-\ell)} \left(x(t-r)\overline{x(t-r-\ell)} - x(t-\hat{r}) \overline{x(t-\hat{r}-\ell)} \right) \right|^2 \\
\end{align}
%
This reveals that the ptychographic likelihood measures a weighted difference between the auto-correlations of the shifted objects $x(t-r)$ and $x(t-\hat{r})$, with the probe-based weight $p(t)\overline{p(t-\ell)}$ which is independent of $r$ and $\hat{r}$.

For general objects $x$ and probe functions $p$, ...

\todo[inline]{SW4TR: did you make any notes for the derivatives you calculated which you could add?}

\todo[inline]{TR@SW: We have the following problem:} let's say $p$ is such the we only consider the contribution at $t=l=0$,  then the above term is basically
%
\begin{align*}
(p(0)\overline{p(0)} (x(-r) \overline{x(-r)} - x(-\hat{r}) \overline{x(-\hat{r})}))^2
\end{align*}
%
which I think is not necessarily convex. Assume everything is real, consider the function $g(r):= (w(-r) - c)^2$, where $c=x^2(-\hat{r})$, $w=x^2$
%
\begin{align*}
d_r g &= -2 (w(-r) - c))\, w'(-r)\\
d_r^2 g &= 2 (w'(-r))^2 + 2 (w(-r) - c) w''(-r).
\end{align*}
%
Note that $w'(-r) = 2 x(-r) x'(-r)$ and 
$w''(-r) = 2 (x'(-r))^2 + 2 x(-r) x''(-r)$. If $x$ is convex, we have $w''\geq 0$. Now for convexity we would need
%
\begin{align*}
(w'(-r))^2 \geq (w(\hat{r})-w(-r)) w''(-r)
\end{align*}
%
If $w(\hat{r})$ is not zero this seems intricate.
\nc


==> sections/91reddiff.tex <==





==> sections/99otheranddeprecated.tex <==











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{View $\Delta$ as latent}
% Here we fit $q_\phi$ only on $p(\cdot|y)$ and view $\Delta$ as latents. This means
% \begin{equation}
%     \min_\phi \mathrm{KL}\left(q_\phi || p(\cdot|y)\right)
% \end{equation}
% where we need to (?) evaluate $p(x|y)$ as:
% \begin{equation}
%     p(x|y) = \int \underbrace{p(x|y,\Delta)}_{(*)} \underbrace{p(\Delta|y)}_{(?)} \mathrm{d}\Delta
% \end{equation}

% The term $(*)$ is tractable via the usual likelihood induced by the forward model and the measurement noise model. The term marked with $(?)$ however is not tractable. Using
% \begin{equation}
%     p(\Delta | y) \propto p(\Delta) p(y|\Delta)
% \end{equation}
% the term $p(y|\Delta)$ is again intractable. Even going to the marginal likelihood (integrated over $x$) does not seem to help us further:
% \begin{equation}
%    p(y|\Delta) = \int p(y|\tilde{x},\Delta) p(\tilde{x}|\Delta) \mathrm{d}\tilde{x}
% \end{equation}
% as again $p(\tilde{x}|\Delta)$ is unavailable (and the integral over all possible images $\tilde{x}$ is also computationally infeasible to begin with).

% \subsection{View $\Delta$ as recovered parameter}
% Here we fit $q_\phi$ on the joint conditional distribution $p(x,\Delta | y)$, which gives us a posterior that allows joint sampling of both $x$ and $\Delta$:
% \begin{equation}
%     \min_\phi \mathrm{KL}(q_\phi || p(x,\Delta | y))
% \end{equation}
% and $(x,\Delta)$ is treated as a jointly recovered variable. This problem is structurally similar to the non-blind formulation. $p(x,\Delta|y)$ can be written as
% \begin{equation}
%     p(x,\Delta|y) \propto p(y|x,\Delta) p(x,\Delta) = p(y|x,\Delta) p(x) p(\Delta)
% \end{equation}
% where the second equality makes the assumption that $p(x)$ and $p(\Delta)$ are independent. This assumption should be well justifiable in various blind problem settings, such as blind deconvolution, imaging through turbulence, or position-blind ptychography: Neither is the true image $x$ ever chosen based on the forward model parameters $\Delta$ nor are the forward model parameters $\Delta$ ever chosen based on the true image $x$.

% In terms of score functions, the above relations also result in nice expressions:
% \begin{align}
%     \nabla_x \log p(x,\Delta|y) &= \nabla_x \log p(y|x,\Delta) + \nabla_x \log p(x) + \underbrace{\nabla_x \log p(\Delta)}_{=0}\\
%     \nabla_\Delta \log p(x,\Delta|y) &= \nabla_\Delta \log p(y|x,\Delta) + \nabla_\Delta \log p(\Delta) + \underbrace{\nabla_\Delta \log p(x)}_{=0}
% \end{align}
% but note that the likelihood scores are once again inaccessible when we involve a diffused $x_t$ in place of $x$, as in Chung et al. \cite{Chung2023Diffusion}. However, we are not using these equations anyway when following the formalism by Feng et al. \cite{Feng2023Score,Feng2024Variational}.

% The joint conditional distribution $p(x,\Delta|y)$ (our posterior) cannot be decomposed into $p(x|y)$ and $p(\Delta|y)$ as these are not mutually independent. Thus, whatever variational distribution we are fitting should be able to represent an actual joint distribution. When using a neural network (such as a normalizing flow) as the variational $q_\phi$, this becomes an architectural problem: DNN architectures are not easily adapted to generically produce an arbitrary-size image $\mathbb{C}^{H\times W}$ \emph{as well as} an arbitrary number of 2D scan positions $\mathbb{R}^{K\times 2}$ at the same time while ensuring good general performance. In particular, note that $K$ has no relation to $H, W$.

% A promising observation is that the later paper by Feng et al. \cite{Feng2024Variational} uses a diagonal-covariance Gaussian to fit the image distribution on a 256x256 MRI image fairly successfully (Fig. 1). Extending such a Gaussian variational distribution to also model $\Delta$ should be straightforward. Co-dependence between $x$ and $\Delta$ could also be achieved by fitting a covariance matrix, at the cost of significant runtime and memory increase. In the case of a circular domain for the positions (crystal), we should probably better fit a multidimensional von Mises distribution on $\Delta$, which also seems doable.


% An open question (for me, Simon) here is how we could theoretically ensure that the process of fitting such an unimodal distribution---when repeated infinitely many times---can faithfully cover the actual posterior with correct mode weights. Something like an ergodicity on the space of the variational probability distributions, viewing $\phi$ as a particle? What properties do our variational distribution $q_\phi$ and our optimizer (and our prior and likelihood?) need to fulfill for this?
% \nc
%%%%%%%%%%%% old exchanges on variational approach %%%%%%%%%%%%
















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section*{Concatenating Diffusion Models and ULA}% older idea by Martin, not pursued further
% Bayes yields 
% $$ p(x|f) = \frac{p(f|x)p_0(x)}{p_0(f)} $$
% and
% $$ \nabla \log p(x|f) = \nabla \log p(f|x) + \nabla \log p_0(x) $$
% The initial samples of the diffusion model are sampled from $p_0$.

% The forward SDE in the diffusion model is given by 
% $$ dX = - \beta(t) X~dt +  \sqrt{2 \beta(t)}~dW, $$
% and the associated probability density $\pi$ solves the Fokker-Planck equation
% $$ \partial_t \pi = \nabla \cdot(\beta x \pi) + \beta \Delta \pi, $$
% and we learn a score $s(x,t) \approx \beta(t) \nabla \log \pi(x,t).$
% The backward process has a density $\rho$ satisfying
% $$ \partial_t \rho = \nabla \cdot(\beta x \rho + 2\rho s) - \beta \Delta \rho, $$

% Ideally we have $u(x) = - \frac{1}{\beta(0)} s(x,0) \approx - \nabla \log p_0(x)$, 
% hence we could simply start a ULA sampling of the posterior by computing
% $$ d\tilde X = u(\tilde X)~dt - \nabla \log p(f|\tilde X)~dt + \sqrt{2}d\tilde W$$
% obvious starting points being the samples obtained from the diffusion process. 

% A remaining problem might be that we cannot control the error between  $s(\cdot,0)$ and $\beta(0) \nabla \cdot p_0$, but only the $L^2$-error in time between $s$ and $\beta \nabla \log \pi$. Alternatives are
% \begin{itemize}
% \item Time averaging: $u(x) = - \frac{1}\tau \int_0^\tau \frac{1}{\beta(t)} s(x,t)~dt$

% \item Learn $u$ from backward samples, e.g. minimize
% $$ \int |u(x) - \frac{2}{\beta(0)} s(x,0) + \nabla \log \rho(x,0)|^2 \rho(x,0)~dx$$
% or
% $$ \int |u(x) - \nabla \log \rho(x,0)|^2 \rho(x,0)~dx = 
% \int ( |u(x)|^2 + 2\nabla \cdot u(x) )  \rho(x,0)~dx+ \text{ const}$$

% \end{itemize}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Regularization by Denoising}

% The original RED paper \cite{Romano2017Little} mainly focuses on solving inverse problems via a regularization approach, i.e.,
% %
% \begin{align*}
% \min_x \frac{1}{2}\|Ax- y\|^2 + \lambda \rho(x).
% \end{align*}
% %
% From a practical side, the authors noticed, that assuming the gradient rule
% %
% \begin{align}\label{eq:red}
% \nabla\rho = x - f(x)
% \end{align}
% %
% where $f$ is some denoiser, leads to a powerful and easy to implement scheme. It was proposed as an alternative to Plug-n-Play methods, and does not require differentiating the denoiser. However, the question what regularizer $\rho$ admits the rule in \eqref{eq:red} is not directly clear. Assuming that the denoiser $f$ is $1$-homogenous and has a symmetric Jacobian one can show that the following regularizer
% %
% \begin{align*}
% \rho(x):= \frac{1}{2}\langle x, x-f(x)\rangle
% \end{align*}
% %
% fulfills the gradient rule. Namely,
% %
% \begin{align*}
% \nabla_x \frac{1}{2} \langle x, x-f(x)\rangle &=
% x - \frac{1}{2} f(x) - \frac{1}{2} J_f(x)^T x\\
% &\overset{(i)}{=}x - \frac{1}{2} f(x) - \frac{1}{2} J_f(x) x\\
% &\overset{(ii)}{=}x - \frac{1}{2} f(x) - \frac{1}{2} f(x)\\
% &= x - f(x),
% \end{align*}
% %
% where in $(i)$ we used the symmetry of the Jacobian, and in $(ii)$ the one-homogeneity of $f$, since
% %
% \begin{gather*}
% \lambda\mapsto h(\lambda) = f(\lambda x) = \lambda f(x)\\
% \Rightarrow
% \frac{d}{d\lambda}h(\lambda) = 
% J_f(\lambda x) x = f(x)\\
% \Rightarrow
% J_f(x) x = f(x).
% \end{gather*}
% %
% In practice one-homogeneity holds true approximately, and locally for many denoisers, which is empirically evaluated in \cite{Romano2017Little}. However, the symmetry of the gradient is usually not fulfilled, which breaks the argumentation above. A more refined description can be found in \cite{Reehorst2019Regularization}. See \cite{Reehorst2019Regularization} section 4 also for an explanation why it might still make sense for denoisers $f$ that do not have symmetric Jacobian, there is an interpretation in terms of matching the score of the prior that $f$ is trained on.
% %
% In \cite{Mardani2024Variational} the authors want to incorporate a score model $\epsilon_\theta$. They derive the following problem
% %
% \begin{align*}
% \min_x \frac{1}{2}\|Ax - y\|^2 +
% \underbrace{\mathbb{E}_{t,\epsilon}\left[
% \|\iota_t (\epsilon_\theta(x_t; t) - \epsilon)\|^2\right]}_{=:\rho(x)}
% \end{align*}
% %
% where $x_t = \alpha_t x + \sigma_t \epsilon$. They then observe that for a specific weighting function (here hidden in $\iota_t$), the gradient of $\rho$ can be computed as follows,
% %
% \begin{align}\label{eq:reddiff}
% \nabla_x \rho(x) = 
% \mathbb{E}_{t,\epsilon}\left[
% \lambda_t (\epsilon_\theta(x_t; t) - \epsilon)\right],
% \end{align}
% %
% which is interesting, since other terms from the chain rule cancel out. Therefore, one does not need to differentiate the score function. 

% \tr
% The step from this to the RED-Diff update now becomes a bit unclear. As far as I understand, the idea is to use gradient in \eqref{eq:reddiff}. At each step one considers the regularizer
% %
% \begin{align*}
% \rho^k(x) := \lambda_t \langle \epsilon(x^{k-1}_t) - \epsilon, x\rangle
% \end{align*}
% %
% which by definition has the desired gradient $\lambda_t(\epsilon(x^{k-1}_t) - \epsilon)$. Other than the fact that $\nabla_x \langle c,x\rangle = x$ for every constant $c$, I don't see the connection to RED.

% \nc

% \textbf{Examining proofs in RED-Diff paper:}\\
% Apart from the question whether there is a variational formulation that is minimized in RED-Diff, let's examine the motivation of the algorithm in a little more detail. Essentially, the proof of Propositions 1 and 2 in the paper break down to writing the Kullback-Leibler divergence in a convenient way and then `hiding' a few things in the reweighting $\omega$.\\
% The approach is parametric, the best approximation to the posterior that we are going to get is $q_0 = N(\mu,\sigma^2 I)$ with some $\mu$ and either $\sigma = 0$ (Dirac and treated as reconstruction instead of sampling) or $\sigma > 0$ (allowing trivial sampling from $q_0$).\\
% Write $ q_t$ and $p_t$ for the diffused versions of $q_0$ and $p_0$ under the typical VP-SDE. We want to minimize $\KL(q_0,p_0)$. This is rewritten in the following convenient way
% \begin{align*}
%     \KL(q_0, p_0) &\approx \KL(q_0, p_0) - \KL(q_T,p_T)\\
%     &= - \left[ \KL(q_t, p_t) \right]_{t=0}^T\\
%     &= - \left[ \omega(t) \KL(q_t, p_t) \right]_{t=0}^T \tag{$\ast$}\\
%     &= - \underbrace{\int_0^T \omega(t) \frac{\mathrm d}{\mathrm d t} \KL(q_t, p_t) \mathrm dt}_{(A)} - \underbrace{\int_0^T \omega'(t) \KL(q_t, p_t) \mathrm dt}_{(B)}
% \end{align*}
% The line $(\ast)$ holds if $\omega(0) = \omega(1) = 1$. Now, the main approach can be summarized as follows:
% \begin{itemize}
%     \item These equations hold true if $\omega$ is $C^1$ with $\omega(0) = \omega(1) = 1$ (say for simplicity $\omega \equiv 1$). If that is the case and the score is exact, then $(B) = 0$ and $(A)$ can be rewritten as a term which the authors call score matching objective. Of course if we want to minimize the posterior KL, we can instead minimize the score matching term. This is Proposition 1.
%     \item We now take a different $\omega$ which has $\omega(0) = 0$. Then instead $(\ast) = 0$. The term $(A)$ is now a weighted score matching objective, but is not related to the $\KL$ of interest anymore of course. Still, we minimize $(A)$. This is simple now using $(A) = - (B)$ and the fact that we can easily compute the gradients $\nabla_\mu, \nabla_\sigma$ of $(B)$ (due to the partial integration, we only get first order $x$-derivatives in $(B)$, which is the reason we don't need to differentiate through the score network). This is Proposition 2.
% \end{itemize}

% Two questions arise at this point: 
% \begin{itemize}
%     \item \textbf{Effect of the reweighting?} We can probably construct quite simply an example in which the wrong $\omega(t)$ leads to the $\KL$ divergence not being minimized. In the paper the implicit choice $\omega'(t) = \lambda \sigma_t^2/\alpha_t^2$ is made, $\omega'(t) \propto e^{2t^2}$. The corresponding $\omega(t)$ has no closed form but explodes really fast of course. Constructing a counterexample might be instructive but not helpful either probably.
%     \item Another potential problem are the instabilities that the authors mention at small $t$: ``We observed that the regularization term in Eq. 9 [i.e. the term under the integral in (A)] is sensitive to noise schedule. For example, in the variance-preserving scenario, it drastically blows up as t approaches zero.'' A reason might be that here we minimize $\KL(q_0,p_0)$ instead of $\KL(p_0,q_0)$. In particular if $p_0$ is singular but we try to fit $q_0$ with $\sigma >0$, then actually $\KL(q_0,p_0) = \infty$ and many of the computations break down. Note that the $\KL$ divergence between two Gaussians is given by 
%     $$\KL(N(\mu_1,\sigma_1^2), N(\mu_2,\sigma_2^2)) = \frac{(\mu_1 - \mu_2)^2 + \sigma_1^2 - \sigma_2^2 }{2\sigma_2^2} + \log(\sigma_2/\sigma_1).$$
% \end{itemize}

% \subsection{Red-Diff algorithm}

% \begin{align*}
% t &\sim \mathcal{U}[0,T]\\
% \epsilon_k &\sim \mathcal{N}(0, I)\\
% %\text{loss} &= \frac{1}{2}\|y- f(\mu)\|^2 + \lambda_t \langle \epsilon_\theta(x_{t-1}; t) - \epsilon, \mu\rangle\\
% x_{k+1}& = \alpha_k \mu_k + \sigma_k \epsilon_k\\
% \mu_{k+1} &= \mu_k - \tau \left(J_f(\mu_k)(f(\mu_k)-y) - \lambda_k(\epsilon_\theta(x_{k+1},k)-\epsilon)\right)\\
% %x_t &= \alpha_t\mu_t + \sigma_t\epsilon \\
% \mathrm d \mu_t &= - \nabla_\mu(\norm{f(\mu_t)-y}^2) - \lambda_t(\epsilon_\theta(\alpha_t\mu_t+\sigma_t\epsilon,t) - \epsilon)\\
% \mathrm d \mu_t &= - \nabla_\mu(\norm{f(\mu_t)-y}^2) - \lambda_t(-\sigma_t\nabla_x p( \mu_t) - \epsilon)\qquad \text{if score exact}
% \end{align*}
